Synthesizing Resilient Strategies for Infinite-Horizon Objectives in Multi-Agent Systems

We consider the problem of synthesizing resilient and stochastically stable strategies for systems of cooperating agents striving to minimize the expected time between consecutive visits to selected locations in a known environment. A strategy profile is resilient if it retains its functionality even if some of the agents fail, and stochastically stable if the visiting time variance is small. We design a novel specification language for objectives involving resilience and stochastic stability, and we show how to efficiently compute strategy profiles (for both autonomous and coordinated agents) optimizing these objectives. Our experiments show that our strategy synthesis algorithm can construct highly non-trivial and efficient strategy profiles for environments with general topology.

==> sections/references-with-arxiv.tex <==
\begin{thebibliography}{}

\bibitem[\protect\citeauthoryear{Almeida \bgroup \em et al.\egroup
  }{2004}]{ARSTMCC:multi-patrolling-survey}
A.~Almeida, G.~Ramalho, H.~Santana, P.~Tedesco, T.~Menezes, V.~Corruble, and
  Y.~Chevaleyr.
\newblock Recent advances on multi-agent patrolling.
\newblock {\em Advances in Artificial Intelligence -- SBIA}, 3171:474--483,
  2004.

\bibitem[\protect\citeauthoryear{Basilico \bgroup \em et al.\egroup
  }{2016}]{BLM:Remote-SW-Protection}
N.~Basilico, A.~Lanzi, and M.~Monga.
\newblock A security game model for remote software protection.
\newblock In {\em Proceedings of {ARES} 2016}, pages 437--443, 2016.

\bibitem[\protect\citeauthoryear{Br{\'{a}}zdil \bgroup \em et al.\egroup
  }{2017}]{BCFK:performance-stability-JCSS}
T.~Br{\'{a}}zdil, K.~Chatterjee, V.~Forejt, and A.~Ku{\v{c}}era.
\newblock Trading performance for stability in {Markov} decision processes.
\newblock {\em Journal of Computer and System Sciences}, 84:144--170, 2017.

\bibitem[\protect\citeauthoryear{Ceccato and
  Tonella}{2011}]{CT:Codebender-IEEESoftware}
M.~Ceccato and P.~Tonella.
\newblock Codebender: Remote software protection using orthogonal replacement.
\newblock {\em IEEE Software}, 28(2):28--34, 2011.

\bibitem[\protect\citeauthoryear{Choset}{2005}]{Choset:book}
H.M.{} Choset.
\newblock {\em Principles of Robot Motion: Theory, Algorithms, and
  Implementation}.
\newblock MIT Press, 2005.

\bibitem[\protect\citeauthoryear{Collberg \bgroup \em et al.\egroup
  }{2012}]{CMMN:distributed-tamper-detection}
C.~Collberg, S.~Martin, J.~Myers, and J.~Nagra.
\newblock Distributed application tamper detection via continuous software
  updates.
\newblock In {\em Proceedings of the 28th Annual Computer Security Applications
  Conference}, pages 319--328. ACM Press, 2012.

\bibitem[\protect\citeauthoryear{Czyzowicz \bgroup \em et al.\egroup
  }{2017}]{CGKKKT:corrupted-patrolmen-Algorithmica}
J.~Czyzowicz, L.~Gasieniec, A.~Kosowski, E.~Kranakis, D.~Krizanc, and N.~Taleb.
\newblock When patrolmen become corrupted: Monitoring a graph using faulty
  mobile robots.
\newblock {\em Algorithmica}, 79:925--940, 2017.

\bibitem[\protect\citeauthoryear{Dixon}{2019}]{Dixon:book}
A.~Dixon.
\newblock {\em Multi-Agent Systems: Design, Synthesis and Analysis}.
\newblock Clanrye International, 2019.

\bibitem[\protect\citeauthoryear{Gronauer and
  Diepold}{2022}]{GD:multiagent-learning-survey}
S.~Gronauer and K.~Diepold.
\newblock Multi-agent deep reinforcement learning: A survey.
\newblock {\em Artificial Intelligence Review}, 55:895--943, 2022.

\bibitem[\protect\citeauthoryear{Hazon and
  Kaminka}{2005}]{HK:robustness-multirobot-ICRA}
N.~Hazon and G.A. Kaminka.
\newblock Redundancy, efficiency and robustness in multi-robot coverage.
\newblock In {\em Proceedings of ICRA 2005}, pages 735--741. IEEE Computer
  Society Press, 2005.

\bibitem[\protect\citeauthoryear{Huang \bgroup \em et al.\egroup
  }{2019}]{HZHH:multi-robot-patrol-survey}
L.~Huang, M.~Zhou, K.~Hao, and E.~Hou.
\newblock A survey of multi-robot regular and adversarial patrolling.
\newblock {\em IEEE/CAA Journal of Automatica Sinica}, 6(4):894--903, 2019.

\bibitem[\protect\citeauthoryear{Kawamura and
  Soejima}{2020}]{KS:Multi-patrol-strategies-TCS}
A.~Kawamura and M.~Soejima.
\newblock Simple strategies versus optimal schedules in multi-agent patrolling.
\newblock {\em Theoretical Computer Science}, 839:195--206, 2020.

\bibitem[\protect\citeauthoryear{Kingma and Ba}{2015}]{Adam}
D.~P. Kingma and J.~Ba.
\newblock Adam: A method for stochastic optimization.
\newblock In {\em Proceedings of {ICLR} 2015}, 2015.

\bibitem[\protect\citeauthoryear{Kla{\v{s}}ka \bgroup \em et al.\egroup
  }{2021}]{KKMR:Regstar-UAI}
D.~Kla{\v{s}}ka, A.~Ku{\v{c}}era, V.~Musil, and V.~{\v{R}}eh{\'{a}}k.
\newblock Regstar: Efficient strategy synthesis for adversarial patrolling
  games.
\newblock In {\em Proceedings of UAI 2021}, pages 471--481, 2021.

\bibitem[\protect\citeauthoryear{Kla{\v{s}}ka \bgroup \em et al.\egroup
  }{2022}]{KKMR:RecReach-IJCAI}
D.~Kla{\v{s}}ka, A.~Ku{\v{c}}era, V.~Musil, and V.~{\v{R}}eh{\'{a}}k.
\newblock General optimization framework for recurrent reachability objectives.
\newblock In {\em Proceedings of the International Joint Conference on
  Artificial Intelligence (IJCAI-ECAI 2022)}, pages 4642--4648, 2022.

\bibitem[\protect\citeauthoryear{Kla{\v{s}}ka \bgroup \em et al.\egroup
	}{2023}]{KKMR:???}
D.~Kla{\v{s}}ka, A.~Ku{\v{c}}era, V.~Musil, and V.~{\v{R}}eh{\'{a}}k.
\newblock Synthesizing Resilient Strategies for Infinite-Horizon Objectives in Multi-Agent Systems.
\newblock {\em arXiv:??? [cs.GT]}, 2023.

\bibitem[\protect\citeauthoryear{LaValle}{2006}]{LaValle:book}
S.M.{} LaValle.
\newblock {\em Planning Algorithms}.
\newblock Cambridge University Press, 2006.

\bibitem[\protect\citeauthoryear{Norris}{1998}]{Norris:book}
J.R.{} Norris.
\newblock {\em {Markov} Chains}.
\newblock Cambridge University Press, 1998.

\bibitem[\protect\citeauthoryear{Paszke \bgroup \em et al.\egroup
	}{2019}]{PyTorch}
A.{} Paszke, S.{} Gross, F.{} Massa, A.{} Lerer, J.{} Bradbury, G.{}
	Chanan, T.{} Killeen, Z.{} Lin, N.{} Gimelshein, L.{} Antiga, A.{}
	Desmaison, A.{} Kopf, E.{} Yang, Z.{} DeVito, M.{} Raison, A.{}
	Tejani, S.{} Chilamkurthy, B.{} Steiner, Lu~Fang, J.{} Bai, and S.{}
	Chintala.
\newblock Pytorch: An imperative style, high-performance deep learning library.
\newblock In {\em Advances in Neural Information Processing Systems 32}, pages
	8024--8035. Curran Associates, Inc., 2019.

\bibitem[\protect\citeauthoryear{Portugal and
  Rocha}{2011}]{PR:multi-patrolling-survey}
D.~Portugal and R.~Rocha.
\newblock A survey on multi-robot patrolling algorithms.
\newblock {\em Technological Innovation for Sustainability}, 349:139--146,
  2011.

\bibitem[\protect\citeauthoryear{Shoham}{2008}]{Shoham:book}
Y.~Shoham.
\newblock {\em Multiagent Systems}.
\newblock Cambridge University Press, 2008.

\bibitem[\protect\citeauthoryear{Sinha \bgroup \em et al.\egroup
  }{2018}]{SFAKT:Stackelberg-Security-Games}
A.~Sinha, F.~Fang, B.~An, C.~Kiekintveld, and M.~Tambe.
\newblock Stackelberg security games: Looking beyond a decade of success.
\newblock In {\em Proceedings of the International Joint Conference on
  Artificial Intelligence (IJCAI 2018)}, pages 5494--5501, 2018.

\bibitem[\protect\citeauthoryear{Smith \bgroup \em et al.\egroup
  }{2011}]{STBR:temporal-planning-IJRS}
S.L.{} Smith, J.~T{\r{u}}mov{\'{a}}, C.~Belta, and D.~Rus.
\newblock Optimal path planning for surveillance with temporal-logic
  constraints.
\newblock {\em International Journal of Robotics Research}, 30(14):1695--1708,
  2011.

\bibitem[\protect\citeauthoryear{Tarjan}{1972}]{Tarjan:SCC-decomp-SICOMP}
R.~Tarjan.
\newblock Depth-first search and linear graph algorithms.
\newblock {\em {SIAM} Journal of Computing}, 1(2), 1972.

\bibitem[\protect\citeauthoryear{Toth and Vigo}{2001}]{TV:book}
P.~Toth and D.~Vigo.
\newblock {\em The Vehicle Routing Problem}.
\newblock SIAM Monographs on Discrete Mathematics and Applications. SIAM, 2001.

\bibitem[\protect\citeauthoryear{van~der Hoek and
  Wooldridge}{2012}]{HW:logics-multiagent-survey}
W.~van~der Hoek and M.~Wooldridge.
\newblock Logics for multiagent systems.
\newblock {\em AI Magazine}, 33(3):92--105, 2012.

\bibitem[\protect\citeauthoryear{Wooldridge}{2009}]{Wooldridge:book}
M.~Wooldridge.
\newblock {\em Introduction to {MultiAgent} Systems}.
\newblock Wiley, 2009.

\bibitem[\protect\citeauthoryear{Yin \bgroup \em et al.\egroup
  }{2010}]{YKKCT:Stackelberg-Nash-security}
Z.~Yin, D.~Korzhyk, C.~Kiekintveld, V.~Conitzer, and M.~Tambe.
\newblock Stackelberg vs.{} {Nash} in security games: Interchangeability,
  equivalence, and uniqueness.
\newblock In {\em Proceedings of AAMAS 2010}, pages 1139--1146, 2010.

\end{thebibliography}

